Applications of a Graph Theoretic Based Clustering Framework in Computer Vision and Pattern Recognition

Recently, several clustering algorithms have been used to solve variety of problems from different discipline. This dissertation aims to address different challenging tasks in computer vision and pattern recognition by casting the problems as a clustering problem. We proposed novel approaches to solve multi-target tracking, visual geo-localization and outlier detection problems using a unified underlining clustering framework, i.e., dominant set clustering and its extensions, and presented a superior result over several state-of-the-art approaches.

==> chapters/summary.tex <==
\chapter*{Preface}
%\lettrine{S}{ummary} goes here.
\lettrine{T}his dissertation presents applications of a graph theoretic clustering framework, namely dominant sets and its variants, in solving problems in computer vision and pattern recognition. Chapter 3 presents the first application of dominant sets to solve tracking problem in a single camera. This led to the first publication \cite{YonEyaPelPraIET2016}. Chapter 4 introduces a new multi-target tracking approach in a multiple non-overlapping camera using constrained dominant sets. This work is under review at Transactions on Pattern Analysis and Machine Intelligence (TPAMI) [the arXiv version is in \cite{YonieyaPAMICDSC_tracker}] and has been developed in the last year of my PhD course, during my second visit to the Center for Research in Computer Vision (CRCV) at University of Central Florida, under the supervision of Dr. Mubarak Shah. Chapter 5 presents a Nobel approach to solve another yet very challenging computer vision problem, i.e., large scale image geo-localization using (constrained) dominant set clustering framework. The result has been published in TPAMI \cite{eyasuPAMIgeoloc}. This work is done during my first visit to CRCV at UCF. Finally, the last chapter of the thesis is devoted to outlier detections, we used some properties of dominant sets to simultaneously solve clustering and outlier detections from data. This work has been presented in \cite{zemene2016simultaneous}.


